Learning to Explore for Stochastic Gradient MCMC

Bayesian Neural Networks(BNNs) with high-dimensional parameters pose a challenge for posterior inference due to the multi-modality of the posterior distributions. Stochastic Gradient MCMC(SGMCMC) with cyclical learning rate scheduling is a promising solution, but it requires a large number of sampling steps to explore high-dimensional multi-modal posteriors, making it computationally expensive. In this paper, we propose a meta-learning strategy to build \gls{sgmcmc} which can efficiently explore the multi-modal target distributions. Our algorithm allows the learned SGMCMC to quickly explore the high-density region of the posterior landscape. Also, we show that this exploration property is transferrable to various tasks, even for the ones unseen during a meta-training stage. Using popular image classification benchmarks and a variety of downstream tasks, we demonstrate that our method significantly improves the sampling efficiency, achieving better performance than vanilla \gls{sgmcmc} without incurring significant computational overhead.

==> tables/augmentation_ood.tex <==
\def\textBF#1{\sbox\CBox{#1}\resizebox{\wd\CBox}{\ht\CBox}{\textbf{#1}}}


\begin{table}[t]
\centering
   \begin{minipage}[t]{0.59\textwidth}
   \centering
   \caption{{Results of image classification with data augmentation.} \vspace{-5pt}} 
   \resizebox{\linewidth}{!}{
     \setlength{\tabcolsep}{3pt}
\begin{tabular}[t]{L{1.7cm}rrrrr}
 \toprule
 Dataset & Method & ACC $\uparrow$ & NLL $\downarrow$ & ECE $\downarrow$  & KLD $\uparrow$ \\


 \midrule
 
\multirow{3}{*}{CIFAR-10}
& \gls{de} & \textbf{0.931}$\spm{0.002}$ & \textbf{0.209}$\spm{0.003}$ &
\textbf{0.017}$\spm{0.001}$ & 0.293$\spm{0.002}$  \\
& \gls{csgmcmc} & 0.923$\spm{0.003}$ & 0.234$\spm{0.007}$ &
0.031$\spm{0.005}$ & 0.142$\spm{0.019}$  \\
& \gls{l2e} & 0.926$\spm{0.001}$ & 0.235$\spm{0.002}$ &
0.037$\spm{0.001}$ & \textbf{0.391}$\spm{0.005}$  \\

 \midrule
 
\multirow{3}{*}{CIFAR-100}
& \gls{de} & \textbf{0.708}$\spm{0.001}$ & \textbf{1.048}$\spm{0.001}$ &
0.092$\spm{0.001}$ & 0.765$\spm{0.003}$  \\
& \gls{csgmcmc} & 0.683$\spm{0.001}$ & 1.114$\spm{0.005}$ &
\textbf{0.013}$\spm{0.001}$ & 0.319$\spm{0.008}$  \\
& \gls{l2e} & 0.705$\spm{0.003}$ & 1.066$\spm{0.001}$ &
0.095$\spm{0.003}$ & \textbf{0.996}$\spm{0.017}$  \\

 \bottomrule
    \end{tabular}} 
\label{tab:exp:clsaug}
   \end{minipage}
   \hspace{1pt}
   \begin{minipage}[t]{.39\linewidth}
   \centering
    \caption{Ablation study on \gls{ood} detection}\vspace{-5pt}
    \resizebox{\linewidth}{!}{
      \setlength{\tabcolsep}{3pt}
        \begin{tabular}[t]{m{1.5cm}rrrr}
        
     \toprule
     In-dist & \gls{ood} & small \gls{l2e} & \gls{l2e}  \\
     \midrule
    \multirow{3}{*}{CIFAR-10}
    & CIFAR-100 &  \textbf{0.855$\spm{0.001}$} & 0.851$\spm{0.001}$ \\
    & SVHN  & 0.929$\spm{0.001}$ & \textbf{0.931$\spm{0.003}$} \\
    & {\scriptsize Tiny-ImageNet} &\textbf{0.855$\spm{0.001}$} & 0.853$\spm{0.001}$\\
     \midrule
    \multirow{3}{*}{CIFAR-100}
    & CIFAR-10  & 0.789$\spm{0.003}$  & \textbf{0.792$\spm{0.002}$} \\
    & SVHN  & 0.912$\spm{0.004}$ & \textbf{0.917$\spm{0.003}$}  \\
    & {\scriptsize Tiny-ImageNet}  & 0.777$\spm{0.001}$ & \textbf{0.782$\spm{0.003}$} \\
     \bottomrule
        \end{tabular}}
\label{tab:exp:oodabl}

\end{minipage}
\end{table} 


==> tables/r.tex <==

\begin{table}[t]
    \centering
     \caption{Proportion of samples with $\hat R < 1.2$.}
     \label{exp:tab:rhat}
     \vskip 0.15in
        \resizebox{\columnwidth}{!}{
        \begin{tabular}{lrrrr}
     \toprule
     \diagbox[width=3.0cm]{Dataset}{Method} & \gls{csgmcmc}  & Meta-\gls{sgmcmc}  & \gls{l2e} 
     % Experiment ($\times 10^5$)  &  \gls{csgmcmc}  & \gls{psgmcmc} & \gls{l2e}  
     \\
     \midrule
    Fashion-MNIST & 0.317 & 0.519  &  \textbf{0.992}   \\
    CIFAR-10 & 0.611 & \textbf{0.975} & 0.920  \\
    CIFAR-100 & 0.584 & \textbf{0.902} & 0.848   \\
    Tiny-ImageNet & 0.679 & 0 & 0.86  \\
     \bottomrule
        \end{tabular}}
     \vskip -0.1in
\end{table}
